Protecting Locations with Differential Privacy under Temporal Correlations

Concerns on location privacy frequently arise with the rapid development of GPS enabled devices and location-based applications. While spatial transformation techniques such as location perturbation or generalization have been studied extensively, most techniques rely on syntactic privacy models without rigorous privacy guarantee. Many of them only consider static scenarios or perturb the location at single timestamps without considering temporal correlations of a moving user's locations, and hence are vulnerable to various inference attacks. While differential privacy has been accepted as a standard for privacy protection, applying differential privacy in location based applications presents new challenges, as the protection needs to be enforced on the fly for a single user and needs to incorporate temporal correlations between a user's locations. In this paper, we propose a systematic solution to preserve location privacy with rigorous privacy guarantee. First, we propose a new definition, "$\delta$-location set" based differential privacy, to account for the temporal correlations in location data. Second, we show that the well known $\ell_1$-norm sensitivity fails to capture the geometric sensitivity in multidimensional space and propose a new notion, sensitivity hull, based on which the error of differential privacy is bounded. Third, to obtain the optimal utility we present a planar isotropic mechanism (PIM) for location perturbation, which is the first mechanism achieving the lower bound of differential privacy. Experiments on real-world datasets also demonstrate that PIM significantly outperforms baseline approaches in data utility.

==> data/locPriv_related.tex <==
\section{Related Work}
Because we have reviewed all mechanisms of differential privacy, in this section we only focus on the related work of location privacy.

There have been many recent work related to location privacy.  Major topics include: spatial transformation of locations, trajectory sharing with privacy protection, privacy preserving query management, and cryptographic approaches
for location sharing.  We classify the closely related work into two fundamental
areas, location privacy preserving mechanisms (LPPMs) and inference (attacks) on location.

\subsection{Location Privacy Preserving Mechanisms and Applications}
Current LPPMs can be roughly classified into two categories. The first is the aggregation based technique, which provides protection for a group of
users. The main idea is to hide a target among a group so that attackers can not distinguish the victim from others. Examples of this type include
k-anonymity \cite{anonymity-attack-09}. % and differentially private \cite{Dwork-dp} trajectory sharing \cite{dp-trajectory-KDD12}.
Many work have demonstrated the vulnerability of anonymization technique.
\cite{anonymity-attack-09} studied the threat of re-identification of anonymous location traces.
The threats is dramatically greater with the disclosure of both home and workplace locations
than either one alone.
\cite{vulnerability-location-10} showed how a third party with some side information can  figure out a user's location in an anonymous trace.
Recently differential privacy has been accepted as a strong mechanism for answering aggregated queries.
\cite{dp-trajectory-KDD12} applied differential privacy to sequential and trajectory data.
Aggregated technique can help on publishing large volume
of trajectory data with personalized privacy guarantee, however, it cannot be used to release a user's data alone for personalized location based service or location sharing without a large group.

The second type is the personalized technique, which protects personal location privacy like this paper. It generally uses some
obfuscation methods, like spatial cloaking, cell merging, location precision reducing or dummy cells, to manipulate the probability distribution of
users' locations. \cite{obfuscation-location-07} proposed the obfuscation technique to express user's privacy preferences on location data.
\cite{obfuscation-framework-06} suggested a framework of using obfuscation technique to provide high quality of location information.
\cite{individual-trajectory-publication-08} studied the problem of publishing a sequence of locations of a moving object considering an adversary who holds partial information about the trajectories.
%It can be shown that these methods mathematically all inject perturbation on probabilities or distributions of a user's location except one method, location hiding, which simply suppresses the release of location if necessary.
%Because of the unexpected situations and the functionalities of devices, like signal problem, weather, dying battery, the probability of hiding location is difficult to calculate.
Based on these mechanisms, location based applications have also been studied.
\cite{kNN-query-obfuscation-VLDB06} solved the query processing, like k-nearest neighbors, for location based services using the obfuscation technique.
\cite{continuous-NN-EDBT09} addressed the problem of processing continuous nearest neighbor queries for moving objects when the exact locations are obfuscated or uncertain.
\cite{events-recommending-ICDM10} carried out a study of recommending
social events from mobile phone location data.
It is obvious that these approaches tried to achieve the optimal tradeoff between the utility of applications and privacy guarantee using the LPPMs.
However, most of these mechanisms do not consider temporal correlations or only apply simple heuristics and therefore are subject to various inference attacks which we will discuss below.



\subsection{Inferences on Location}
Various inference attacks can be carried out based on location information and external information such as moving patterns.  These include: re-identification of a user,
location disclosure of a user, probabilistic privacy breach of certain types of information such as presence in an area, trajectory during certain period, and so on.
Several work showed (re)identification attacks based on location information.
\cite{geo-identifier} evaluated the risk of re-identifying a user even if the user identity is not explicitly released because
the geo-localized history of user-requests can act as a quasi-identifier. % and may be used to access sensitive information.
\cite{geo-idenfication-2008} showed how to identify a user from the records of cellular network based on previous movements.
\cite{trace-attack2} conducted an inference attack against obfuscation techniques and showed that a small fraction of users can be identified
and home addresses of a big fraction of users were exposed.

Other works attempted to infer a user's actual location through modeling user's mobility and to define how to quantify location privacy (not just the identity). 
\cite{Quantifying-location-privacy-SP2011} investigated the question of how to formally quantify the privacy of existing LPPMs.  An adversary can model users' mobility using a Markov process learned from a population.  %It defined the privacy by the probability of disclosure. Then by formalizing the adversary's performance, it calculated the privacy with the proposed metrics
It then clarified three metrics related to location inference including accuracy, certainty and correctness, and argued the last one should be used as a privacy metric.  
\cite{Liao-learning-pattern} used a hierarchical Markov model to learn and infer a user's trajectory based on the places and temporal patterns they visited.  \cite{putmode_Qiao10} used the Continuous Time Bayesian Networks to predict uncertain trajectories of moving objects.
\cite{Xue_ICDE13} proposed a Sub-Trajectory Synthesis algorithm to learn the transition matrix of Markov chain and to predict a user's destination.
Although these work were not in the context of privacy protection, the inspiration to us is that we should also assume adversaries have the ability to learn user's moving pattern and make the
inference. This is why we use the strong adversary model against what differential privacy privacy is guaranteed.
Complicated inferences, like spatio-temporal queries, can also be derived with matrix computations. % which extended location query processing to the realm of stochastic process.
With the Markov model and uncertain locations of moving objects, \cite{Querying-ST-ICDE12} proposed a modified matrix computation method to efficiently compute the probability of a user appearing in certain region during certain time period.



In conclusion, location privacy has received a lot of attention. Although many LPPMs and related inference attacks have been proposed, they either did not protect a reliable privacy or proposed other adversary models which are not so trustworthy. 
To our knowledge, none of existing work
has provided differential privacy in the presence of the strong adversary who can model a user's mobility through a Markov process. Because correlation is the key characteristic of geospatial data,
differential privacy has to be extended to handle correlations.

